Cabbage: A Differential Growth Framework for Open Surfaces

We propose Cabbage, a differential growth framework to model buckling behavior in 3D open surfaces found in nature-like the curling of flower petals. Cabbage creates high-quality triangular meshes free of self-intersection. Cabbage-Shell is driven by edge subdivision which differentially increases discretization resolution. Shell forces expands the surface, generating buckling over time. Feature-aware smoothing and remeshing ensures mesh quality. Corrective collision effectively prevents self-collision even in tight spaces. We additionally provide Cabbage-Collision, and approximate alternative, followed by CAD-ready surface generation. Cabbage is the first open-source effort with this calibre and robustness, outperforming SOTA methods in its morphological expressiveness, mesh quality, and stably generates large, complex patterns over hundreds of simulation steps. It is a source not only of computational modeling, digital fabrication, education, but also high-quality, annotated data for geometry processing and shape analysis.

==> ICCV2025-Author-Kit-Feb/sec/v0-Results.tex <==
% % Vertex Count for Cabbage
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel={Simulation Step},
%         ylabel={\# Vertices},
%         title={Number of Vertices},
%         grid=both,
%         width=8.5cm,
%         height=6cm,
%         legend pos=north west
%     ]
%     \addplot[
%         color=red,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,  
%         x=time,         
%         y=value         
%     ] {Stats/data.csv};  
%     \addlegendentry{$D^2$}
    
%     \addplot[
%         color=blue,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value
%     ] {Stats/morb-v-ct.csv};
%     \addlegendentry{$\mathbb{M}$}

%     \addplot[
%         color=green,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value
%     ] {Stats/ring-v-ct.csv};
%     \addlegendentry{$S^1 \times I$}

%     \addplot[
%         color=orange,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value
%     ] {Stats/putr-v-ct.csv}; 
%     \addlegendentry{$T^2 \backslash D^2$}
    
%     \end{axis}

% \end{tikzpicture}

% % Triangle Quality for Cabbage
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel={Simulation Step},
%         ylabel={Triangle Quality},
%         title={Triangle Quality},
%         grid=both,
%         width=8.5cm,
%         height=6cm,
%         legend pos=north west,
%         error bars/y dir=both,
%         error bars/y explicit
%     ]
    
%     \addplot[
%         color=blue,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value,
%         y error=std
%     ] {Stats/emyu-q-mean-std.csv};
%     \addlegendentry{Cabbage}

%     \end{axis}

% \end{tikzpicture}

% % Dihedral for Cabbage
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel={Simulation Step},
%         ylabel={Mean Sq. Dihedral Angle},
%         title={Dihedral Angles},
%         grid=both,
%         width=8.5cm,
%         height=6cm,
%         legend pos=north west,
%     ]
    
%     \addplot[
%         color=blue,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value,
%         y error=std
%     ] {Stats/emyu-dihedral.csv};
%     \addlegendentry{Cabbage}

%     \end{axis}

% \end{tikzpicture}

% % Valence for Cabbage
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel={Simulation Step},
%         ylabel={Avg. Valence},
%         title={Valence},
%         grid=both,
%         width=8.5cm,
%         height=6cm,
%         legend pos=north west,
%     ]
    
%     \addplot[
%         color=blue,
%         mark=*,
%         mark size=1.2pt
%     ] table [
%         col sep=comma,
%         x=step,
%         y=value,
%         y error=std
%     ] {Stats/emyu-valence.csv};
%     \addlegendentry{Cabbage}

%     \end{axis}

% \end{tikzpicture}
\input{Stats/cabbage-stats}

\input{Stats/user-study}

\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
    \setlength{\tabcolsep}{2pt} % Adjust column spacing if needed
    \begin{tabular}{lccccc}
        \toprule
        & \% Self-Crossing & \% Failure & Face Quality & Dihedral Angle$^2$ & Valence \\
        \midrule
        A & --  & --  & --  & --  & --  \\
        B & --  & --  & --  & --  & --  \\
        C & --  & --  & --  & --  & --  \\
        D & --  & --  & --  & --  & --  \\
        E & --  & --  & --  & --  & --  \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of different metrics across five cases (A–E).}
    \label{tab:comparison}
\end{table}

\section{Experiments}
\subsection{Dataset and Evaluation Metric} We compare Cabbage to Yu \cite{EmYu}, Okunskiy \cite{Okunskiy}, Horikawa \cite{Horikawa}, and Bachman \cite{Bachman} which are the only methods with reproducible implementations to the best of our knowledge. We evaluate these methods on dataset of $120$ randomly-generated meshes equally distributed over three homeomorphic types of 3D open surfaces: Disk $D^2$, Annulus (Ring, $S^1 \times I$), a Möbius Band, and a Punctured Torus ($T^2 \backslash D^2$). Due to the distinct properties of the methods we compare, the resulting mesh from running a constant number of iterations can vary greatly. Therefore, we instead set a goal of $3,000$ vertices beyond which we stop the simulation. For the experiments, we record the occurrence of self-intersection events, growth failure, and distince morphological development. We also conduct a user study in Tab~\ref{tab:user-study} to meter the real-world effectiveness of Cabbage. 

\subsection{Quantitative Results}
In the first few steps of the simulation, modifications to the same initial mesh is similar. After that, the methods' striking diversity becomes apparent. 

\textit {Growth Speed} The mesh size of Horikawa grows quickly over time due to repeated remeshing from a coarse base mesh with a short target length. The mesh size of collision-driven approaches (Yu, Bachman, Okunskiy) grows the fastest over time. In contrast, mesh size grows in a steady, controlled manner with Cabbage whilst buckling pattern emerge and develop.

\noindent \textbf{Vertex Degree Distribution} With additional edges being created, the absence of edge flips in Okunskiy and Bachman leads to high valence. Horikawa's global remeshing ensures relatively uniform valence. Edge flips in Yu and Cabbage limits valence. Valence is further reduced by edge collapses in Cabbage.

\noindent \textbf{Face Quality} Very sharp triangles in Okunskiy even with large smoothing strength due to the lack of topology update, especially at high-curvature areas, which limits the ability of collision responses to prevent self-intersections. Horikawa's isotropic remeshing per iteration ensured mesh triangle quality. Edge length and vertex collision constraints in Bachman similarly preserve the shape of faces. In Yu, collision, edge flips, and barycentric smoothing after each simulation step maintains face quality but its differential application from scaling the smoothing vectors by growth rates works poorly when areas with low growth rates buckle. This is exacerbated by the optimization to skip collision responses vertices with low growth rates.

Cabbage-Shell's stretch forces ensure that edge lengths converge toward $L_0$, while ODT smoothing ensures isotropism even in actively growing areas with high curvature. Edge flips, collapses, and the removal of ears further clean up the mesh as it deforms. Cabbage-Collision improves on Yu by decoupling smoothing and growth factor distribution, ensuring face quality throughout the mesh.

\noindent \textbf{Self-Intersection} The dual purpose of collision responses in Yu and Bachman to create buckling and prevent self-intersection has limited effectiveness in crowded areas as discussed in Sec~ \ref{sec:self-intersection}. The increased jaggedness at the boundary edges and the large dihedral angles in Bachman intensify this issue. The usage of spherical colliders is a limitation for Okunskiy, as long edges in degenerate triangles effectively leave 'gaps' in the mesh surface that should overwise be fully 'covered' by the colliders' surface, leading to self-intersections. 

Cabbage-Shell and Cabbage-Collision's corrective collision is dedicated specifically to detecting preventing self-collision after vertex position has been adjusted by growth forces. This ensures that there is no cross-contamination of the corrective collision forces by forces that serve purposes other than to prevent self-collision. Meanwhile, the ellipsoidal colliders that adapt to local mesh geometry (which by the nature of differential growth can have short or long edges) as well as additional smoothing of these collision forces in Cabbage-Shell ensures stability and accuracy.

\noindent \textbf{Mesh Smoothness}\label{sec:smoothness} The disparity in mesh smoothness across the compared methods highlight the choice of smoothing and the supervising role of bending forces. Okunskiy's mesh is highly jagged from the onset. In Bachman, smoothness is maintained only prior to buckling; as the mesh size increase rapidly, it quickly becomes jagged, especially at open boundaries. We note that while subdivision such as \cite{LoopSubdivision} can create a smooth experience, the coarse base mesh greatly limits the range of possible curved profile of the morphology. Horikawa faces a similar tradeoff: while global remeshing and laplacian smoothing are effective measures in principle, the base mesh which is perturbed randomly leads to crumpled, wrinkly surface. We note additionally that due to the nature of Horikawa's global remeshing, vertices from the mesh prior to remeshing do not remain. This leads to a jittering appearance as the mesh develops over time.

Cabbage and Yu's lead in smoothness metric highlight the importance of buckling formation on a smooth mesh with sufficient resolution. While Yu achieves this through barycentric smoothing, enhancing smoothness by increasing the strength of this smoothing attenuates local details that could otherwise develop into large buckling the algorithm aims to achieve. Cabbage's bending forces is an additional separate layer of smoothing that contributes to the buckling process, and it is complemented by the feature-preserving quality of ODT smoothing.

\subsection{Qualitative Results} 
We conduct a user study of $83$ domain experts and students in fine art, 3d art, and digital fabrication to evaluate Cabbage against the aforementioned methods in the dimensions of aesthetic quality, shape exploration potential, conduciveness to further design and modification, and manufacturability. Our metrics are the task completion time, SUS score $(0\text{–}100)$, NASA-TLX $(0\text{–}100)$, and an aesthetic rating $(0\text{–}7)$. 

\noindent \textbf{Aesthetics and Morpological Range}. While retaining excellent mesh quality, Cabbage-Shell exhibit a very wide range of potential shapes and versatility over various initial conditions. On the one hand, the distribution of growth factors provide another dimension of control for the differential behavior of growth. Bachman and Horikawa does not have this. Bachman's morphology initially differs but inevitably converges into a large bush with small leaves. Horikawa does not split the mesh but rather rely on the isotropic remeshing following the random displacement of the vertices of the base mesh to generate additional geometry. This leads to a very large and wrinkly mesh with only global-scale buckling. Okunskiy enabled user-defined assignment of vertex weight in the Blender user interface, greatly expanding the shape space, but the lack of mesh quality limits realism and aesthetics. Yu's method generates both global and local buckling in a smooth manner, enhancing realism and aesthetics. However, both are limited by mesh smoothness and nuanced control of buckling development (see Sec~\ref{sec:smoothness}). Cabbage overcome these challenges, mesh smoothness and quality are maintained whilst the scale of buckling could be intuitively adjusted with the bending stiffness parameter.

\noindent \textbf{Design and Fabrication} The practical value of Cabbage is enhanced by its ability to prevent self-intersections even as the mesh grows very large ($1 \times 10^5$) vertices as well as the CAD conversion pipeline which retains its shape in a lightweight and editable format. Though this approach (see Sec~\ref{sec:CAD-conversion}) is applicable to many triangular meshes, including those from methods we compared to, it is particularly effective on meshes generated by Cabbage and Yu due to their smoothness and resolution. For coarse-grain meshes whose buckling areas has large dihedral angles, algorithmically discerning these sharp features from the curved forms they are meant to represent in the quad remeshing process becomes challenging. We note that the CAD-conversion capability is very helpful for the intricate shape generated by Cabbage as manually creating (and then offsetting) such complex surfaces is highly labor-intensive.

\subsection{Ablation}
\noindent \textit{Effect of Growth Factor Distribution} Growth cutoff has a large impact on morphology because buckling occur at areas of high growth factors. This is especially the case when growth factors are a considerable geodesically spaced-out. With a low steepness value and sparse growth factors, the area of the mesh close to a growth factor quickly moves away from that of another growth factor, creating elongated forms. But this also limits the area of the mesh with high growth, hence buckling. Meanwhile, a high steepness value provides ample area for buckling to appear, though we find that $0.5$ is often sufficient. In our experiments, we use a steepness value of $0.5$; it has little impact on the morphology.

\noindent \textit{Effect of Bending Force} As buckling develop, bending forces play a critical role in ensuring the mesh's smoothness in a feature-preserving manner. But a bending force coefficient high enough to achieve this would inhibit out-of-plane behavior early in the simulation, greatly delaying the emergence of buckling. Our solution is to vary the bending coefficient over time, starting with a very small value before increasing to that sufficient to maintain mesh smoothness. The advent of buckling is greatly hastened, especially when the initial mesh is planar.

\noindent \textit{Effect of Initial Surface} The final morphology of the surface varies greately not only from the initial morphology of the mesh but also its topology. We observe that the range of parameters that lead to stable growth is much larger for initial meshes that are already nearly isotropic and 5-6-7. Though the valence of newly-generated meshes vertices are optimized toward a desired 5-6-7, high-valence vertices in the initial mesh may persist.

